On the Detection of Mutual Influences and Their Consideration in Reinforcement Learning Processes

Self-adaptation has been proposed as a mechanism to counter complexity in control problems of technical systems. A major driver behind self-adaptation is the idea to transfer traditional design-time decisions to runtime and into the responsibility of systems themselves. In order to deal with unforeseen events and conditions, systems need creativity -- typically realized by means of machine learning capabilities. Such learning mechanisms are based on different sources of knowledge. Feedback from the environment used for reinforcement purposes is probably the most prominent one within the self-adapting and self-organizing (SASO) systems community. However, the impact of other (sub-)systems on the success of the individual system's learning performance has mostly been neglected in this context. In this article, we propose a novel methodology to identify effects of actions performed by other systems in a shared environment on the utility achievement of an autonomous system. Consider smart cameras (SC) as illustrating example: For goals such as 3D reconstruction of objects, the most promising configuration of one SC in terms of pan/tilt/zoom parameters depends largely on the configuration of other SCs in the vicinity. Since such mutual influences cannot be pre-defined for dynamic systems, they have to be learned at runtime. Furthermore, they have to be taken into consideration when self-improving the own configuration decisions based on a feedback loop concept, e.g., known from the SASO domain or the Autonomic and Organic Computing initiatives. We define a methodology to detect such influences at runtime, present an approach to consider this information in a reinforcement learning technique, and analyze the behavior in artificial as well as real-world SASO system settings.

==> Inputs/300-delayed-influences-eval-figures.tex <==
\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/DistanceCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/DistanceCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the distance correlation with one estimator.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{distance correlation}. For this measurement only a \textbf{single estimator} has been used, i.e., the configurations of  workbench $B_{RU}$ have not been considered.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_no-own-config_distance-correlation}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/MaximalInformationReshefCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/MaximalInformationReshefCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the maximal information coefficient with one estimator.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Maximal Information Coefficient}. For this measurement only a \textbf{single estimator} has been used, i.e., the configurations of  workbench $B_{RU}$ have not been considered.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_no-own-config_mic}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/MutualInformationKraskovCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/MutualInformationKraskovCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the continuous mutual information with one estimator.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Continuous Mutual Information}. For this measurement only a \textbf{single estimator} has been used, i.e., the configurations of  workbench $B_{RU}$ have not been considered.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_no-own-config_continuous-mutual-information}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/OnlineKendallCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/OnlineKendallCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the Kendall rank correlation with one estimator.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Kendall rank correlation}. For this measurement only a \textbf{single estimator} has been used, i.e., the configurations of  workbench $B_{RU}$ have not been considered.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_no-own-config_kendall}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/OnlineMutualInformationDiscreteCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/OnlineMutualInformationDiscreteCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the discrete mutual information with one estimator.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Discrete Mutual Information}. For this measurement only a \textbf{single estimator} has been used, i.e., the configurations of  workbench $B_{RU}$ have not been considered.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_no-own-config_discrete-mutual-information}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/PearsonCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/PearsonCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the Pearson correlation coefficient with one estimator.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Pearson correlation coefficient}. For this measurement only a \textbf{single estimator} has been used, i.e., the configurations of  workbench $B_{RU}$ have not been considered.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_no-own-config_pearson-correlation}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/SpearmanCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/no-own-config/SpearmanCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the Spearman rank correlation with one estimator.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Spearman rank correlation}. For this measurement only a \textbf{single estimator} has been used, i.e., the configurations of  workbench $B_{RU}$ have not been considered.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_no-own-config_spearman}
\end{figure}
\afterpage{\clearpage}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/DistanceCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/DistanceCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the distance correlation with two estimators.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{distance correlation}. For this measurement \textbf{two estimators} have been used, i.e., the configurations of  workbench $B_{RU}$ have been taken into account.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_with-own-config_distance-correlation}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/MaximalInformationReshefCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/MaximalInformationReshefCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the maximal information coeffcient with two estimators.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Maximal Information Coefficient}. For this measurement \textbf{two estimators} have been used, i.e., the configurations of  workbench $B_{RU}$ have been taken into account.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_with-own-config_mic}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/MutualInformationKraskovCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/MutualInformationKraskovCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the continuous mutual information with two estimators.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Continuous Mutual Information}. For this measurement \textbf{two estimators} have been used, i.e., the configurations of  workbench $B_{RU}$ have been taken into account.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_with-own-config_continuous-mutual-information}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/OnlineKendallCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/OnlineKendallCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the Kendall rank correlation with two estimators.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Kendall rank correlation}. For this measurement \textbf{two estimators} have been used, i.e., the configurations of workbench $B_{RU}$ have been taken into account.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_with-own-config_kendall}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/OnlineMutualInformationDiscreteCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/OnlineMutualInformationDiscreteCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the discrete mutual information with two estimators.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Discrete Mutual Information}. For this measurement \textbf{two estimators} have been used, i.e., the configurations of  workbench $B_{RU}$ have been taken into account.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_with-own-config_discrete-mutual-information}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/PearsonCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/PearsonCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the Pearson correlation coefficient with two estimators.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Pearson correlation coefficient}. For this measurement \textbf{two estimators} have been used, i.e., the configurations of  workbench $B_{RU}$ have been taken into account.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_with-own-config_pearson-correlation}
\end{figure}
\afterpage{\clearpage}

\begin{figure}	
	\centering
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/SpearmanCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneCorrectDetectionRate.pdf}
		\caption{The fraction of 100 runs in which the influence has been detected as higher than a notional independent workbench for each delay in time steps.}		
	\end{subfigure}
	\\
	\begin{subfigure}[t]{\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/eval/industry/simple/with-own-config/SpearmanCalculator/P1UPPER-P2UPPER/P1UPPER-P2UPPER-AllInOneMiRate.pdf}
		\caption{The averaged influence values.}
	\end{subfigure}
\caption[The results for the smart factory application using the Spearman rank correlation with two estimators.]{The results for the smart factory application. The graphs show the results for the influence of the upper workbench at the left station $B_{LU}$ on the upper workbench on the right station $B_{RU}$ measured with the \textbf{Spearman rank correlation}. For this measurement \textbf{two estimators} have been used, i.e., the configurations of  workbench $B_{RU}$ have been taken into account.}\label{fig:300-detection-of-influences_further-aspects_delayed-influences_simple_with-own-config_spearman}
\end{figure}
\afterpage{\clearpage}
